Scalable Hash Table for NUMA Systems

Hash tables are used in a plethora of applications, including database operations, DNA sequencing, string searching, and many more. As such, there are many parallelized hash tables targeting multicore, distributed, and accelerator-based systems. We present in this work a multi-GPU hash table implementation that can process keys at a throughput comparable to that of distributed hash tables. Distributed CPU hash tables have received significantly more attention than GPU-based hash tables. We show that a single node with multiple GPUs offers roughly the same performance as a 500-1,000-core CPU-based cluster. Our algorithm's key component is our use of multiple sparse-graph data structures and binning techniques to build the hash table. As has been shown individually, these components can be written with massive parallelism that is amenable to GPU acceleration. Since we focus on an individual node, we also leverage communication primitives that are typically prohibitive in distributed environments. We show that our new multi-GPU algorithm shares many of the same features of the single GPU algorithm -- thus we have efficient collision management capabilities and can deal with a large number of duplicates. We evaluate our algorithm on two multi-GPU compute nodes: 1) an NVIDIA DGX2 server with 16 GPUs and 2) an IBM Power 9 Processor with 6 NVIDIA GPUs. With 32-bit keys, our implementation processes 8B keys per second, comparable to some 500-1,000-core CPU-based clusters and 4X faster than prior single-GPU implementations.

==> single-gpu.tex <==
% We first introduce single-GPU HashGraph.
% Our intuition behind HashGraph is to treat hashing in terms of graphs.
% We have a set of vertices corresponding to keys, and a set of vertices corresponding to all possible hash values.
% Between these two sets of vertices, each edge connects a key to the hash value for that key.
% The result is HashGraph is a bipartite graph between keys and hash values.
% This interpretation lets HashGraph leverage a unique set of benefits.
% One of the more obvious benefits is HashGraph can use much of the research in graph optimizations, since at the end of the day, it is simply a graph.
% \todo{This is an example of fluff in this section. Can simplify / get rid of this}
% On top of this, HashGraph offers a ``best-of-both-worlds'' option in terms of hashing.
% Most hash tables ultimately boil down to one of two categories: 1) separate chaining and 2) open addressing.
% \todo{I can be more brief on this. I'll explain OA/Chaining hashing in the background}.
% With separate chaining, we can quickly lookup keys with the same hash value.
% However, we store these keys as a linked lists, which have a number of scalability issues.
% Open addressing is, in some sense, the inverse.
% Hash tables with open addressing cannot look exclusively at keys with the same hash value.
% As a result, lookups often involve a lot more work, as we need to sift through a larger number of keys.
% However, open addressing also uses arrays over linked lists.
% Hash tables with open addressing can then scale a lot easier than those with separate chaining.
% HashGraph manages to keep the benefits of both chaining and open addressing, while avoiding the demerits of each.
% Since it is a bipartite graph between keys and their hash values, HashGraph lets us look exclusively at keys with a particular hash value.
% This benefit was only there for separate chaining.
% % On top of this, we can implement HashGraph with arrays since we can implement graphs with arrays (in particular, with the CSR format discussed later).
% Together, HashGraph has all the benefits of both chaining and open addressing yet manages to avoid their downsides.

% HashGraph is also a \textit{static} hash table.
% This means that all the keys in the hash table must be inputted when the table is constructed, and it is not possble to add or delete keys after the table is built.
% This differs from \textit{dynamic} hash tables, which do permit $add$ and $delete$ operations.
% \todo{Can probably have a bit more of a transition between here and storing HG}

% In order to discuss how to build a HashGraph, we must first describe how it is stored.
% Recall that HashGraph is a bipartite graph.
% Naturally, we store HashGraph with a common sparse-graph data structure.
% Our implementation uses the \textit{Compressed Sparse Row} (CSR) structure.

% \subsection{Storing HashGraph as CSR}
% % For our internal representation of HashGraph, we use \textit{Compressed-Sparse Row (CSR)}.
% CSR implements an adjacency list for a graph with two arrays instead of linked lists.
% One array, $edges$ of length $|E|$, includes all the neighbors in the graph.
% % That is, the first $deg(v_0)$ elements in $edges$ are the neighbors of vertex $v_0$, the next $deg(v_1)$ are the neighbors of $v_1$, and so on.
% We also have an array $offset$ of length $|V|$.
% % The $offset$ array has an entry per vertex, each pointing to the first neighbor of that vertex in $edges$.
% Concretely, $offset[i]$ points to the first neighbor of $v_i$ in $edges$, and the next $deg(v_i)$ elements in $edges$ are $v_i$'s neighbors.
% % Together, this means that the elements in $edges[offset[i] \ldots offset[i] + deg(v_i)]$ are exactly the neighbors of $v_i$.
% Note also that $deg(v_i)$ is simply $offset[i + 1] - offset[i]$.
% Figure \ref{fig:csr} is a CSR representation for the example graph.
% In the context of HashGraph, our $edges$ array has length $N$ and our $edges$ array has length $N / C$.
% \todo{Might discuss CSR in Background. Delete this section if so.}
% 
% \begin{figure}[t!]
%     \centering
%     \includegraphics[scale=0.3]{figures/csr_fig.pdf}
%     \caption{CSR Representation of Example Graph}
%     \label{fig:csr}
% \end{figure}

As described above, HashGraph stores all of its data as a bipartite graph. 
Our implementation of HashGraph stores backing graph in a CSR representation.
Thus, building a HashGraph is identical to building the backing CSR.

\subsection{Building HashGraph}
At its core, building a HashGraph is just building both the $offset$ and $edges$ arrays described above.
These are the only two arrays in a CSR representation, so these are the only two arrays in HashGraph.

% NOTE: These two subsubsections might get into too much detail. Comes off as just describing the pseudocode.
% NOTE: Need to talk about LRB at some point.

\subsubsection{Constructing $offset$}
% Recall that the $offset$ array is of length $|V|$, and each entry $offset[i]$ points to the neighbors of vertex $v_i$.
Recall that $offset[i + 1] - offset[i] = deg(v_i)$, and $v_i$ corresponds to a hash value.
We can construct the $offset$ array in two steps: 1) create an array with the degree of each hash, and 2) prefix sum this array.
Note that the degree of a hash is just the number of keys with that hash value.
We can determine this number for each hash in parallel, using the first three parallel \texttt{for}-loops of Algorithm \ref{alg:sg-hg-build}.
After this computation, we can simply run a prefix sum.
The result is the $offset$ array for HashGraph.

% Recall that each $v_i$ corresponds to a hash value $h_i$.
% Because of this, computing $deg(v_i)$ is simply counting the number of keys that hash to $h_i$.
% Naturally, we can first hash each key in parallel.
% The first \texttt{for}-loop in Algorithm \ref{alg:sg-hg-build} depicts this, storing the hashes in array $H_A$.
% After hashing each key, we can iterate over each hash value in parallel, and tally the number of instances of each hash value.
% Our pseudocode in Algorithm \ref{alg:sg-hg-build} does this with the second and third \texttt{for}-loops.
% We, essentially, increment $counter[H_A[i]]$ for each $i$ in parallel.
% Once $counter$ is populated, we can simply run a $prefix\_sum$ operation on this array, and the return value is the $offset$ array for HashGraph.

\begin{algorithm}
\caption{Single-Node HashGraph Build. Note $V = N / C$ \cite{greenHashgraph2019}}
\begin{algorithmic}[1]
\ParFor{$i = 0, \ldots, N - 1$}
    \State $H_A[i] = hash(A[i]) \mod V$
\EndParFor
\ParFor{$i = 0, \ldots, V - 1$}
    \State $CounterArray[i] = 0$
\EndParFor
\ParFor{$i = 0, \ldots, N - 1$}
    \State $AtomicAdd(CounterArray[H_A[i]], 1)$
\EndParFor
\State $offset = PrefixSum(CounterArray)$
\ParFor{$i = 0, \ldots, V - 1$}
    \State $CounterArray[i] = 0$
\EndParFor
\ParFor{$i = 0, \ldots, N - 1$}
    \State $pos = AtomicAdd(CounterArray[H_A[i]], 1)$
    \State $edges[pos + offset[H_A[i]]] = A[i]$
\EndParFor
\end{algorithmic}
\label{alg:sg-hg-build}
\end{algorithm}

\subsubsection{Constructing $edges$}
Recall that, with $edges$, we must have $edges[offset[i]]$ be the first neighbor of $v_i$.
We can leverage the now-computed $offset$ array to populate the $edges$ array as well.
The last parallel \textit{for}-loop in Algorithm \ref{alg:sg-hg-build} illustrates this process.
We simply compute the hash of each key $i$, and insert it into $edges[offset[hash(i)]]$ with counters.
% Recall that the $edges$ array contains every key sorted by hash value.
% To construct the $edges$ array, we have an array of counters of length $|V|$, initialized to $0$.
% For this, we can reuse $counter$ from above.
% We can iterate over each key in parallel once more, and add each key to $edges[offset[H_A[i]] + counter[H_A[i]]$.
% After each addition, we atomatically increment $counter[H_A[i]]$.
% Because $offset[i]$ points to the index of the first key in $edges$, we ensure that there will be no conflicting writes to the same index in $edges$.
% Algorithm \ref{alg:sg-hg-build} illustrates this step in the last two \texttt{for}-loops.
% We have no constructed both the $offset$ and $edges$ arrays for the CSR of HashGraph, thus completely building an instance of HashGraph.

% NOTE: Should also mention cache locality wrt lists.
\subsection{Querying HashGraph}
% Querying a HashGraph for a set of keys is also an efficient operation.
Hash tables also require a \textit{query} operation, where a user can efficiently look up a separate set keys in the table.
HashGraph also supports efficient querying.
Note that we can construct another HashGraph from the keys we wish to look up.
This gives us two total HashGraphs: one with the original set of keys, and one with the keys we want to look up.
From here, we can intersect the list of keys for a particular hash value between both HashGraphs.
The result of such an intersection, across all possible hash values, are the keys to look up that exist in the original HashGraph.
Furthermore, these intersections can be done in parallel, as shown in Algorithm \ref{alg:sg-hg-inter}.
% Let $K_A$ be the set of input keys to the HashGraph, and $K_B$ the set of keys to lookup.
% Also let $HG_A$ be the HashGraph built from $K_A$.
% After constructing $HG_A$, there are two main steps in the querying phase: 1) build another HashGraph from $K_B$ called $HG_B$ and 2) intersect $HG_A$ with $HG_B$.
% We can build $HG_B$ with the same HashGraph build algorithm.
% Intersecting $HG_A$ with $HG_B$ is also not complex.
% This can be done by intersecting the keys associated with some particular hash value in both $HG_A$ and $HG_B$, for all possible hash values.
% If a key exists in $HG_A$, it would exist in $HG_B$ under the same hash value.
% Algorithm \ref{alg:sg-hg-inter} depicts this operation.
% Note two observations here.
% First, we can iterate over all hash values in parallel on a GPU, as the lists of keys for each hash value are disjoint.
% Second, we can lookup keys with a particular hash value efficiently, as established above.
% Putting these two points together, we can lookup a set of keys in a HashGraph by essentially doing a large number of small list intersections in parallel.

\begin{algorithm}
\caption{Single-Node HashGraph Intersect. Note $V = N / C$ \cite{greenHashgraph2019}}
\begin{algorithmic}[1]
\State $HG_A = HashGraph(A, N_A, V)$
\State $HG_B = HashGraph(B, N_B, V)$
\ParFor{$i = 0, \ldots, V - 1$}
    \State $IntersectArray(HG_A[i], HG_B[i])$
\EndParFor
\end{algorithmic}
\label{alg:sg-hg-inter}
\end{algorithm}

